Entropic Riemannian Neural Optimal Transport

Many machine learning problems involve data supported on curved spaces such as spheres, rotation groups, hyperbolic spaces, and general Riemannian manifolds, where Euclidean geometry can distort distances, averages, and the resulting optimal transport (OT) problem. Existing manifold OT methods have pursued amortized out-of-sample maps, while entropic regularization has made discrete OT more scalable, but these advantages have remained largely disjoint. We propose Entropic Riemannian Neural Optimal Transport (Entropic RNOT), a unified framework that combines intrinsic entropic OT with amortized out-of-sample evaluation on Riemannian manifolds. Our method learns a single target-side Schr\"odinger potential through a neural pullback parameterization, recovers the induced Gibbs coupling, and uses the resulting conditional laws to construct intrinsic transport surrogates. These include barycentric projections on Cartan-Hadamard manifolds and heat-smoothed conditional surrogates on stochastically complete manifolds, the latter turning possibly atomic target laws into absolutely continuous ones. For fixed regularization $\varepsilon>0$, we prove that the proposed hypothesis class recovers the entropic optimal coupling in strong probabilistic metrics. As consequences, barycentric surrogates converge in $L^2$, while heat-smoothed surrogates are stable at fixed heat time and asymptotically unbiased as the heat time vanishes. The guarantees hold for compactly supported data on possibly noncompact manifolds. Empirically, our method matches or improves over Euclidean, tangent-space, and log-Euclidean baselines on benchmarks over $\mathbb{S}^2$, $\mathrm{SO}(3)$, $\mathrm{SPD}(3)$, $\mathrm{SE}(3)$, and $\mathbb{H}^2$, scales favorably relative to discrete manifold Sinkhorn, and in a protein-ligand docking application, refines poses on $\mathrm{SE}(3)$ without retraining or per-instance optimization.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sections/app-entropic-transport-kernels.tex <==
\subsection{Entropic transport kernels and deterministic surrogates}
\label{app:entropic-kernel}

This subsection records a useful interpretation of the fixed-temperature
entropic coupling as a probability-valued transport rule. At positive
temperature \(\varepsilon>0\), the canonical transport object is not in general
a deterministic map, but rather a conditional distribution over target points
given each source point.

\begin{definition}[Entropic transport kernel]
\label{def:entropic-transport-kernel}
Let \(M\) be a compact Riemannian manifold, let \(c:M\times M\to\mathbb R\) be
a continuous cost, and let \(\mu,\nu\in\mathcal P(M)\). Fix
\(\varepsilon>0\), and let \((f_\varepsilon,g_\varepsilon)\) be entropic dual
potentials such that the corresponding entropic optimal plan
\(\pi_\varepsilon\in\Pi(\mu,\nu)\) has Gibbs form
\[
\pi_\varepsilon(dx,dy)
=
\exp\!\left(
\frac{f_\varepsilon(x)+g_\varepsilon(y)-c(x,y)}{\varepsilon}
\right)\mu(dx)\nu(dy).
\]
The associated \emph{entropic transport kernel}
\(Q_\varepsilon:M\to\mathcal P(M)\) is defined by
\[
Q_\varepsilon(x,dy)
:=
\exp\!\left(
\frac{f_\varepsilon(x)+g_\varepsilon(y)-c(x,y)}{\varepsilon}
\right)\nu(dy).
\]
Equivalently, using only the semidual potential \(g_\varepsilon\),
\[
Q_\varepsilon(x,dy)
=
\frac{
\exp\!\left(\frac{g_\varepsilon(y)-c(x,y)}{\varepsilon}\right)
}{
\int_M
\exp\!\left(\frac{g_\varepsilon(z)-c(x,z)}{\varepsilon}\right)\nu(dz)
}\,\nu(dy).
\]
\end{definition}

The next proposition states that \(Q_\varepsilon(x,\cdot)\) is precisely the
conditional law of the entropic coupling given the source point \(x\), and that
it pushes \(\mu\) exactly to \(\nu\).

\begin{proposition}[Exact pushforward by the entropic kernel]
\label{prop:exact-pushforward-entropic-kernel}
Under the assumptions of
Definition~\ref{def:entropic-transport-kernel}, the following hold.

\begin{enumerate}
\item
For \(\mu\)-a.e.\ \(x\in M\), \(Q_\varepsilon(x,\cdot)\) is a probability
measure on \(M\).

\item
The entropic coupling disintegrates as
\[
\pi_\varepsilon(dx,dy)=\mu(dx)\,Q_\varepsilon(x,dy).
\]

\item
The kernel \(Q_\varepsilon\) pushes \(\mu\) exactly to \(\nu\), in the sense
that for every Borel set \(B\subset M\),
\[
\nu(B)=\int_M Q_\varepsilon(x,B)\,\mu(dx).
\]
Equivalently, if \(Q_{\varepsilon\#}\mu\) denotes the pushforward of \(\mu\) by
the probability-valued map \(x\mapsto Q_\varepsilon(x,\cdot)\), then
\[
Q_{\varepsilon\#}\mu=\nu.
\]
\end{enumerate}
\end{proposition}

\begin{proof}
Since \(\pi_\varepsilon\) has first marginal \(\mu\), we have for
\(\mu\)-a.e.\ \(x\),
\[
\int_M
\exp\!\left(
\frac{f_\varepsilon(x)+g_\varepsilon(y)-c(x,y)}{\varepsilon}
\right)\nu(dy)
=1.
\]
Hence \(Q_\varepsilon(x,\cdot)\) is a probability measure for \(\mu\)-a.e.\ \(x\),
which proves (1). The identity
\[
\pi_\varepsilon(dx,dy)=\mu(dx)\,Q_\varepsilon(x,dy)
\]
is immediate from the definition, so (2) holds.

Finally, let \(B\subset M\) be Borel. Using that \(\pi_\varepsilon\) has second
marginal \(\nu\), we obtain
\[
\int_M Q_\varepsilon(x,B)\,\mu(dx)
=
\int_M\int_M \mathbf 1_B(y)\,Q_\varepsilon(x,dy)\,\mu(dx)
=
\int_{M\times M}\mathbf 1_B(y)\,\pi_\varepsilon(dx,dy)
=
\nu(B).
\]
This proves (3).
\end{proof}

\begin{remark}[Stochastic analogue of a transport map]
\label{rem:finite-temperature-analogue-monge}
For fixed \(\varepsilon>0\), the natural transport object is the
probability-valued map
\[
x\longmapsto Q_\varepsilon(x,\cdot)\in\mathcal P(M),
\]
rather than a deterministic map \(M\to M\). Equivalently, \(Q_\varepsilon\)
defines the Markov operator
\[
(P_\varepsilon\varphi)(x):=\int_M \varphi(y)\,Q_\varepsilon(x,dy),
\qquad \varphi\in C(M),
\]
whose adjoint acts on measures by
\[
P_\varepsilon^\ast\mu=\nu.
\]
Thus, at positive temperature, the exact finite-temperature analogue of Monge
transport is a stochastic kernel.
\end{remark}

\begin{remark}[Deterministic summaries are only surrogates]
\label{rem:deterministic-surrogates}
Any deterministic pointwise summary extracted from \(Q_\varepsilon(x,\cdot)\),
such as a barycentric projection, a maximum-a-posteriori choice,
or the exponential-gradient proxy
\[
T_\varepsilon(x)=\exp_x\bigl(-\nabla f_\varepsilon(x)\bigr),
\]
is in general only a surrogate for the entropic transport and need not satisfy
\[
(T_\varepsilon)_\#\mu=\nu.
\]
The exact marginal constraint is carried by the full kernel
\(Q_\varepsilon(x,\cdot)\), not by a deterministic collapse to a single point.
\end{remark}

\begin{remark}[Evaluation of the kernel]
\label{rem:evaluation-entropic-kernel}
Writing
\[
Q_\varepsilon(x,dy)
=
\frac{
\exp\!\left(\frac{g_\varepsilon(y)-c(x,y)}{\varepsilon}\right)
}{
Z_\varepsilon(x)
}\,\nu(dy),
\qquad
Z_\varepsilon(x)
:=
\int_M
\exp\!\left(\frac{g_\varepsilon(z)-c(x,z)}{\varepsilon}\right)\nu(dz),
\]
evaluating \(Q_\varepsilon(x,\cdot)\) at a fixed source point \(x\) amounts to
computing the Gibbs score
\[
s_x(y):=\frac{g_\varepsilon(y)-c(x,y)}{\varepsilon}
\]
together with the normalizing constant \(Z_\varepsilon(x)\).

If the target measure is discrete,
\[
\nu=\sum_{j=1}^N b_j\,\delta_{y_j},
\qquad
b_j\ge 0,
\qquad
\sum_{j=1}^N b_j=1,
\]
then
\[
Q_\varepsilon(x,\{y_j\})
=
\frac{
b_j \exp\!\left(\frac{g_\varepsilon(y_j)-c(x,y_j)}{\varepsilon}\right)
}{
\sum_{k=1}^N
b_k \exp\!\left(\frac{g_\varepsilon(y_k)-c(x,y_k)}{\varepsilon}\right)
},
\]
so evaluation reduces to a softmax over the target atoms, with cost \(O(N)\)
per source point once the values \(g_\varepsilon(y_j)\) are available.

If \(\nu\) is continuous, then evaluating \(Q_\varepsilon(x,\cdot)\) requires
approximating the normalizing integral \(Z_\varepsilon(x)\) and related
expectations under \(Q_\varepsilon(x,\cdot)\). Standard approaches include
quadrature, Monte Carlo sampling, importance sampling, and local asymptotic
approximations when \(\varepsilon\) is small. For instance, given samples
\(y_1,\dots,y_N\sim \nu\), one may approximate
\[
Q_\varepsilon(x,\cdot)
\approx
\sum_{j=1}^N w_j(x)\,\delta_{y_j},
\qquad
w_j(x)
=
\frac{
\exp\!\left(\frac{g_\varepsilon(y_j)-c(x,y_j)}{\varepsilon}\right)
}{
\sum_{k=1}^N
\exp\!\left(\frac{g_\varepsilon(y_k)-c(x,y_k)}{\varepsilon}\right)
},
\]
which again reduces evaluation to a softmax over sampled target points.
\end{remark}

\begin{remark}[Point-valued outputs require an additional choice]
\label{rem:transported-value-positive-temperature}
At positive temperature, the entropic transport does not canonically assign a
single target point to a source point \(x\). The canonical transported object is
the conditional probability measure
\[
Q_\varepsilon(x,\cdot)\in\mathcal P(M).
\]
To obtain a point-valued output, one must impose an additional selection rule.

A first possibility is to sample
\[
Y_\varepsilon \mid X=x \sim Q_\varepsilon(x,\cdot).
\]
If \(X\sim\mu\), then \(Y_\varepsilon\sim\nu\), so this is the exact
finite-temperature transport mechanism.

A second possibility is a maximum-a-posteriori selection,
\[
T_\varepsilon^{\mathrm{MAP}}(x)
\in
\arg\max_{y\in M}
\bigl\{
g_\varepsilon(y)-c(x,y)
\bigr\},
\]
which is deterministic but does not in general satisfy
\[
(T_\varepsilon^{\mathrm{MAP}})_\#\mu=\nu.
\]

A third possibility is to use a moment-based summary such as a barycenter.
Such deterministic summaries may be useful computationally, but they remain
surrogates for the full kernel and do not preserve the target marginal in
general.
\end{remark}

==> sections/barycenter-computations.tex <==
\subsection{Intrinsic barycentric projection of the entropic plan on Cartan--Hadamard manifolds}

Let $(\mathcal M,g)$ be a Cartan--Hadamard manifold, i.e.\ a complete, simply connected Riemannian manifold with non-positive sectional curvature. In particular, $(\mathcal M,d)$ is a Hadamard (equivalently, global NPC) space. Hence, for every probability measure $q\in\mathcal P_2(\mathcal M)$, the Fr\'echet functional
\[
z\longmapsto \int_{\mathcal M} d(z,y)^2\,q(dy)
\]
is strictly convex and admits a unique minimizer. This allows one to define the barycenter map
\[
\operatorname{bar}(q)
:=
\argmin_{z\in\mathcal M}
\int_{\mathcal M} d(z,y)^2\,q(dy).
\]

Now let $\pi_\varepsilon^\star\in\Pi(\mu,\nu)$ denote the entropically regularized optimal coupling between $\mu$ and $\nu$, and let
\[
\pi_\varepsilon^\star(dx,dy)=\mu(dx)\,\pi_{\varepsilon,x}^\star(dy)
\]
be its disintegration with respect to the first marginal. Since $\pi_\varepsilon^\star$ is, in general, a diffuse coupling rather than a Monge map, it does not canonically define a deterministic transport map. On a Cartan--Hadamard manifold, however, one obtains a canonical deterministic representative by taking the barycenter of each conditional measure:
\[
T_\varepsilon(x)
:=
\operatorname{bar}(\pi_{\varepsilon,x}^\star),
\qquad x\in \operatorname{supp}(\mu).
\]
Equivalently,
\[
T_\varepsilon(x)
=
\argmin_{z\in\mathcal M}
\int_{\mathcal M} d(z,y)^2\,\pi_{\varepsilon,x}^\star(dy).
\]
We refer to $T_\varepsilon$ as the \emph{intrinsic entropic barycentric projection} of the entropic optimizer.

\paragraph{First-order characterization.}
For fixed $x$, define
\[
\Phi_x(z)
:=
\frac12\int_{\mathcal M} d(z,y)^2\,\pi_{\varepsilon,x}^\star(dy).
\]
Since $\mathcal M$ is Cartan--Hadamard, the function $\Phi_x$ is geodesically strictly convex, and its unique minimizer is $T_\varepsilon(x)$. Using the identity
\[
\nabla_z \Big(\frac12 d(z,y)^2\Big) = -\log_z(y),
\]
one obtains the first-order optimality condition
\[
\nabla \Phi_x(z)
=
-\int_{\mathcal M} \log_z(y)\,\pi_{\varepsilon,x}^\star(dy).
\]
Therefore $z=T_\varepsilon(x)$ if and only if
\[
\int_{\mathcal M} \log_{T_\varepsilon(x)}(y)\,\pi_{\varepsilon,x}^\star(dy)=0.
\]
This equation is the intrinsic analogue of the Euclidean condition that the centered first moment vanishes.

\subsubsection{Discrete entropic barycentric projection}

In practice, one typically approximates the target measure by a discrete measure
\[
\hat\nu
=
\sum_{j=1}^K \alpha_j \delta_{y_j},
\qquad
\alpha_j>0,
\qquad
\sum_{j=1}^K \alpha_j=1.
\]
For the entropic problem with cost $c(x,y)=\frac12 d(x,y)^2$, the conditional law of the discrete entropic optimizer takes the Gibbs form
\[
\pi_{\varepsilon,x}^\star
=
\sum_{j=1}^K w_j^\varepsilon(x)\,\delta_{y_j},
\]
where
\[
w_j^\varepsilon(x)
=
\frac{\alpha_j \exp\!\big((\psi_\varepsilon(y_j)-c(x,y_j))/\varepsilon\big)}
{\sum_{\ell=1}^K \alpha_\ell \exp\!\big((\psi_\varepsilon(y_\ell)-c(x,y_\ell))/\varepsilon\big)}.
\]
If the empirical target is uniform, i.e.\ $\alpha_j=1/K$, this reduces to the softmax formula
\[
w_j^\varepsilon(x)
=
\frac{\exp\!\big((\psi_\varepsilon(y_j)-c(x,y_j))/\varepsilon\big)}
{\sum_{\ell=1}^K \exp\!\big((\psi_\varepsilon(y_\ell)-c(x,y_\ell))/\varepsilon\big)}.
\]

The corresponding intrinsic barycentric projection is then
\[
T_\varepsilon(x)
=
\argmin_{z\in\mathcal M}
\frac12\sum_{j=1}^K w_j^\varepsilon(x)\,d(z,y_j)^2.
\]
Again, since $\mathcal M$ is Cartan--Hadamard, this minimizer is unique. Its first-order condition is
\[
\sum_{j=1}^K w_j^\varepsilon(x)\,\log_{T_\varepsilon(x)}(y_j)=0.
\]
Thus, the intrinsic entropic barycentric map is characterized as the unique zero of the vector field
\[
G(x,z)
:=
\sum_{j=1}^K w_j^\varepsilon(x)\,\log_z(y_j)
\in T_z\mathcal M.
\]
That is,
\[
G\bigl(x,T_\varepsilon(x)\bigr)=0.
\]

\paragraph{Remark on the distinction with extrinsic projection.}
A commonly used surrogate in embedded manifolds is
\[
\widetilde T_\varepsilon(x)
=
\operatorname{proj}_{\mathcal M}\!\left(\sum_{j=1}^K w_j^\varepsilon(x)\,y_j\right),
\]
where the average is taken in the ambient Euclidean space and $\operatorname{proj}_{\mathcal M}$ denotes an ambient projection back to the manifold. This construction is generally \emph{not} equal to the intrinsic barycenter
\[
T_\varepsilon(x)
=
\argmin_{z\in\mathcal M}\frac12\sum_{j=1}^K w_j^\varepsilon(x)\,d(z,y_j)^2,
\]
except in flat situations where the intrinsic and ambient geometries coincide. In particular, on curved manifolds the intrinsic barycentric projection must be defined through the Fr\'echet minimization problem above.

\subsubsection{Computation by Karcher iteration}

A natural numerical scheme for computing $T_\varepsilon(x)$ is the Riemannian gradient descent (or Karcher flow)
\[
z^{(m+1)}
=
\exp_{z^{(m)}}\!\left(
\eta_m
\sum_{j=1}^K w_j^\varepsilon(x)\,\log_{z^{(m)}}(y_j)
\right),
\]
where $\eta_m>0$ is a step size. Indeed, if one sets
\[
\Phi_x(z)
=
\frac12\sum_{j=1}^K w_j^\varepsilon(x)\,d(z,y_j)^2,
\]
then
\[
\nabla \Phi_x(z)
=
-\sum_{j=1}^K w_j^\varepsilon(x)\,\log_z(y_j),
\]
so the iteration above is precisely gradient descent for $\Phi_x$. On a Cartan--Hadamard manifold, the objective is geodesically convex, and the iteration converges to the unique minimizer under standard step-size conditions.

\subsubsection{Differential of the intrinsic barycentric map}

If one is interested in the Jacobian of $T_\varepsilon$ (for instance, in change-of-variables formulas or KL divergence computations), the intrinsic formulation also admits an implicit differentiation formula. Since
\[
G\bigl(x,T_\varepsilon(x)\bigr)=0,
\]
the implicit function theorem yields
\[
dT_\varepsilon(x)
=
-\bigl(D_z G(x,T_\varepsilon(x))\bigr)^{-1}
D_x G(x,T_\varepsilon(x)),
\]
provided $D_z G(x,T_\varepsilon(x))$ is invertible. Here,
\[
G(x,z)=\sum_{j=1}^K w_j^\varepsilon(x)\,\log_z(y_j),
\]
so the derivative splits into two contributions:
\[
D_x G(x,z)
=
\sum_{j=1}^K \bigl(D_x w_j^\varepsilon(x)\bigr)\,\log_z(y_j),
\]
and
\[
D_z G(x,z)
=
\sum_{j=1}^K w_j^\varepsilon(x)\,D_z\!\bigl(\log_z(y_j)\bigr).
\]
This gives the intrinsic Jacobian of the entropic barycentric projection and is the appropriate manifold counterpart of differentiating an explicit Euclidean barycentric map.

\subsubsection{Simplifications on specific manifolds}

The intrinsic barycentric projection simplifies substantially on some manifolds of interest.

\paragraph{Euclidean space.}
If $\mathcal M=\mathbb R^d$, then
\[
\log_z(y)=y-z,
\qquad
\exp_z(v)=z+v,
\]
and the barycentric condition becomes
\[
\sum_{j=1}^K w_j^\varepsilon(x)\,(y_j-T_\varepsilon(x))=0.
\]
Hence
\[
T_\varepsilon(x)=\sum_{j=1}^K w_j^\varepsilon(x)\,y_j.
\]
Thus, in Euclidean space the intrinsic barycenter coincides with the ordinary weighted average.

\paragraph{The manifold of symmetric positive definite matrices with the affine-invariant metric.}
Let $\mathcal M=\mathrm{SPD}(n)$ endowed with the affine-invariant Riemannian metric. The intrinsic barycenter of matrices $Y_1,\dots,Y_K\in \mathrm{SPD}(n)$ with weights $w_1,\dots,w_K$ is the unique minimizer of
\[
X\longmapsto \frac12\sum_{j=1}^K w_j\,\delta_{\mathrm{AI}}(X,Y_j)^2,
\]
where
\[
\delta_{\mathrm{AI}}(X,Y)
=
\left\|
\log\!\bigl(X^{-1/2}YX^{-1/2}\bigr)
\right\|_F.
\]
The first-order condition becomes
\[
\sum_{j=1}^K w_j\,
\log\!\bigl(X^{-1/2}Y_jX^{-1/2}\bigr)=0.
\]
Equivalently, using the Riemannian logarithm
\[
\log_X(Y)
=
X^{1/2}\log\!\bigl(X^{-1/2}YX^{-1/2}\bigr)X^{1/2},
\]
the barycenter equation is
\[
\sum_{j=1}^K w_j\,\log_X(Y_j)=0.
\]
In general there is no closed form for $K\geq 3$, but the manifold is Cartan--Hadamard and the Karcher iteration applies directly. For two matrices, the weighted barycenter is the weighted geometric mean
\[
X = Y_1 \#_t Y_2
:=
Y_1^{1/2}\bigl(Y_1^{-1/2}Y_2Y_1^{-1/2}\bigr)^t Y_1^{1/2},
\qquad t\in[0,1].
\]

\paragraph{The SPD manifold with the log-Euclidean metric.}
If $\mathrm{SPD}(n)$ is instead equipped with the log-Euclidean metric, then the matrix logarithm is an isometry from $\mathrm{SPD}(n)$ onto the vector space of symmetric matrices. In this case, the intrinsic barycenter has the explicit formula
\[
X
=
\exp\!\left(
\sum_{j=1}^K w_j \log Y_j
\right).
\]
Thus the entropic barycentric projection is obtained by taking the Euclidean weighted average in logarithmic coordinates and exponentiating back to $\mathrm{SPD}(n)$.

\paragraph{Hyperbolic space.}
Let $\mathcal M=\mathbb H^n$ be hyperbolic space. The barycentric projection is again the unique minimizer of
\[
z\longmapsto \frac12\sum_{j=1}^K w_j\,d_{\mathbb H}(z,y_j)^2.
\]
There is generally no closed-form expression for $K\geq 3$, but the intrinsic characterization remains
\[
\sum_{j=1}^K w_j\,\log_z(y_j)=0.
\]
Hence one may compute the hyperbolic barycenter by the same Karcher iteration
\[
z^{(m+1)}
=
\exp_{z^{(m)}}\!\left(
\eta_m \sum_{j=1}^K w_j\,\log_{z^{(m)}}(y_j)
\right).
\]
For two points, however, the weighted barycenter reduces to the geodesic interpolation
\[
z = \exp_{y_1}\!\bigl(t\,\log_{y_1}(y_2)\bigr),
\qquad t\in[0,1].
\]
Thus hyperbolic space admits explicit simplifications at the level of $\exp$ and $\log$, even though a general closed form for the Fr\'echet mean is not available.

\subsubsection{Summary}

The key point is that, on a Cartan--Hadamard manifold, the entropic coupling $\pi_\varepsilon^\star$ admits a canonical deterministic representative through intrinsic barycentric projection:
\[
T_\varepsilon(x)
=
\operatorname{bar}(\pi_{\varepsilon,x}^\star).
\]
In the discrete setting,
\[
T_\varepsilon(x)
=
\argmin_{z\in\mathcal M}
\frac12\sum_{j=1}^K w_j^\varepsilon(x)\,d(z,y_j)^2,
\]
with weights $w_j^\varepsilon(x)$ given by the discrete Gibbs formula. The resulting map is characterized by the intrinsic stationarity condition
\[
\sum_{j=1}^K w_j^\varepsilon(x)\,\log_{T_\varepsilon(x)}(y_j)=0,
\]
and can be computed by Riemannian gradient descent / Karcher flow. This is the geometrically correct manifold analogue of the Euclidean entropic barycentric projection.

==> sections/old_theoretical_guarantees.tex <==
We now introduce the class of neural semidual potentials used to parameterize
entropic transport plans. The key point is that, in the semidual formulation,
only the Schr\"odinger potential \(g\) on \(K_\nu\) is parameterized explicitly,
while the companion potential \(f\) is recovered through the soft
\(c\)-transform.

Recall from Section~\ref{sec:gdl-background} that \(\mathcal F\) is dense in
\(C(\mathbb R^n,\mathbb R)\) under the ucc topology. Let
\[
\varphi:K_\nu\to\mathbb R^n
\]
be a feature map satisfying Assumption~\ref{ass-feature-regularity}, and let
\(\varphi^*\mathcal F\) denote the pullback class introduced in
\eqref{eq-pullback-class-definition}. By the transfer principle from
Section~\ref{sec:gdl-background}, the class \(\varphi^*\mathcal F\) is dense in
\(C(K_\nu)\) under \(\|\cdot\|_{L^\infty(K_\nu)}\).

The Schr\"odinger potentials are defined only up to the additive transformation
\[
(f,g)\mapsto (f-a,g+a),\qquad a\in\mathbb R.
\]
Thus one must choose a normalization in order to single out a representative.
Since we work in the semidual formulation, it is natural to normalize the
\(g\)-potential by requiring zero \(\nu\)-mean:
\[
\int_{K_\nu} g\,d\nu=0.
\]
This is only a choice of representative within the same equivalence class and
does not affect the induced Gibbs plan.

To encode this constraint, define the centering operator
\[
\mathsf C_\nu h
:=
h-\int_{K_\nu} h\,d\nu,
\qquad h\in C(K_\nu),
\]
and the centered pullback class
\[
\mathcal G
:=
\mathsf C_\nu(\varphi^*\mathcal F)
=
\{\mathsf C_\nu a:\ a\in \varphi^*\mathcal F\}
\subset C(K_\nu).
\]
By construction, every \(g\in\mathcal G\) satisfies
\[
\int_{K_\nu} g\,d\nu=0.
\]

For any measurable \(g:K_\nu\to\mathbb R\) such that
\(\mathcal T_\nu^\varepsilon g\) is finite, define the associated Gibbs measure
\begin{equation}
\label{eq:neural-gibbs-plan}
d\pi_g^\varepsilon(x,y)
:=
\exp\!\left(
\frac{\mathcal T_\nu^\varepsilon g(x)+g(y)-c(x,y)}{\varepsilon}
\right)\,d\mu(x)d\nu(y).
\end{equation}

The next result shows that the centered pullback class \(\mathcal G\) is rich
enough to approximate the normalized entropic Schr\"odinger potential and hence
to recover the entropic optimal plan.

\begin{theorem}[Recovery of the entropic optimal plan from approximate semidual maximizers]
\label{thm:recovery-entropic-plan}
Assume that \(\mathcal F\subset C(\mathbb R^n,\mathbb R)\) is dense under the
ucc topology and that the feature map \(\varphi:K_\nu\to\mathbb R^n\) satisfies
Assumption~\ref{ass-feature-regularity}. Then there exists a sequence
\((g_m)_{m\in\mathbb N}\subset \mathcal G\) such that
\[
\mathcal J_\varepsilon(g_m)\xrightarrow[m\to\infty]{}\mathrm{OT}_\varepsilon,
\qquad
\mathrm{KL}(\pi_\varepsilon^\star\mid \pi_{g_m}^\varepsilon)\xrightarrow[m\to\infty]{}0,
\qquad
\|\pi_{g_m}^\varepsilon-\pi_\varepsilon^\star\|_{\mathrm{TV}}\xrightarrow[m\to\infty]{}0.
\]
In particular,
\[
\pi_{g_m}^\varepsilon\rightharpoonup \pi_\varepsilon^\star.
\]
\end{theorem}

The proof is given in Appendix~\ref{app-proof-recovery-entropic-plan}.Next we pass to the zero-regularization limit. For \(\varepsilon>0\) and
\(g\in \mathcal G\), set
\[
f_g^\varepsilon:=\mathcal T_\nu^\varepsilon g,
\]
and define the associated neural Gibbs plan by
\begin{equation}
\label{eq:neural-gibbs-plan-diagonal}
d\pi_g^\varepsilon(x,y)
:=
\exp\!\left(
\frac{f_g^\varepsilon(x)+g(y)-c(x,y)}{\varepsilon}
\right)\,d\mu(x)d\nu(y).
\end{equation}

Under the standing assumptions of Section~\ref{sec:eot-compact-supports},
the supports \(K_\mu\) and \(K_\nu\) are compact and
\[
c(x,y)=\frac12 d(x,y)^2
\]
is continuous on \(K_\mu\times K_\nu\). In particular, the unregularized
optimal transport problem admits at least one optimal plan, and every weak
accumulation point of the entropic optimal plans as \(\varepsilon\downarrow0\)
is an optimal transport plan. We now show that the same is true for a suitable
diagonal family of neural Gibbs plans.

\begin{theorem}[Diagonal recovery of optimal transport plans]
\label{thm:diagonal-plan}
Assume the hypotheses of Theorem~\ref{thm:recovery-entropic-plan}, and let
\((\varepsilon_k)_{k\in\mathbb N}\) be any sequence such that
\(\varepsilon_k\downarrow0\). Then there exists a sequence
\((g_k)_{k\in\mathbb N}\subset \mathcal G\) such that, with
\[
\Delta_k:=\mathrm{OT}_{\varepsilon_k}-\mathcal J_{\varepsilon_k}(g_k),
\]
we have
\[
\frac{\Delta_k}{\varepsilon_k}\xrightarrow[k\to\infty]{}0.
\]

Moreover, the family \((\pi_{g_k}^{\varepsilon_k})_{k\in\mathbb N}\) is
relatively compact for weak convergence, and every weak accumulation point is
an optimal plan for the unregularized quadratic transport problem between
\(\mu\) and \(\nu\).

If, in addition, the unregularized quadratic optimal transport problem admits a
unique optimal plan
\[
\pi^\star\in\Pi(\mu,\nu),
\]
then
\[
\pi_{g_k}^{\varepsilon_k}\rightharpoonup \pi^\star
\qquad\text{as }k\to\infty.
\]
In particular, since \(K_\mu\times K_\nu\) is compact,
\[
W_1\!\left(\pi_{g_k}^{\varepsilon_k},\pi^\star\right)\xrightarrow[k\to\infty]{}0.
\]
\end{theorem}

The proof of Theorem~\ref{thm:diagonal-plan} is postponed to
Appendix~\ref{app-proof-thm-diagonal-plan}.


\begin{remark}
In Theorem~\ref{thm:diagonal-plan}, no separate existence assumption on the
unregularized optimal plan is needed: existence is automatic under the standing
compact-support assumptions. The uniqueness assumption is used only to upgrade
subsequence convergence to convergence of the full diagonal sequence.
\end{remark}
\paragraph{Recovering the OT Map on Cartan Hadamard Manifolds.}



\begin{theorem}[Neural recovery of the entropic barycentric map]
\label{thm:neural-recovery-entropic-map}
Assume the hypotheses of Theorem~\ref{thm:plan-convergence}. Then, for each fixed
$\varepsilon>0$,
\[
\widehat\pi_{m,\varepsilon}\to \pi_\varepsilon^\star
\quad\text{in total variation},
\]
and
\[
\widehat T_{m,\varepsilon}\to T_\varepsilon
\quad\text{in }L^1(\mu)\text{ and }L^2(\mu).
\]
More precisely,
\[
\int d\bigl(\widehat T_{m,\varepsilon},T_\varepsilon\bigr)\,d\mu
\le
D_\nu\sqrt{\frac{\Delta_{m,\varepsilon}}{2\varepsilon}},
\qquad
\int d\bigl(\widehat T_{m,\varepsilon},T_\varepsilon\bigr)^2\,d\mu
\le
D_\nu^2\sqrt{\frac{\Delta_{m,\varepsilon}}{2\varepsilon}}.
\]
\end\subsection{Cartan--Hadamard barycentric projection and recovery of transport maps}
\label{sec:ch-barycentric-projection}

In this subsection we specialize to the case where \((\mathcal M,g)\) is a
Cartan--Hadamard manifold, i.e.\ a complete, simply connected Riemannian manifold
with nonpositive sectional curvature. We retain the notation of
Section~\ref{sec:eot-compact-supports}: the measures \(\mu,\nu\in\mathcal P(\mathcal M)\)
have compact supports
\[
K_\mu:=\operatorname{spt}(\mu),
\qquad
K_\nu:=\operatorname{spt}(\nu),
\]
the cost is
\[
c(x,y):=\frac12 d(x,y)^2,
\]
and, for each \(\varepsilon>0\), the entropic optimal plan is denoted by
\(\pi_\varepsilon^\star\) with Schr\"odinger potentials
\((f_\varepsilon^\star,g_\varepsilon^\star)\).

We further write
\[
D_\nu:=\operatorname{diam}(K_\nu)<\infty,
\qquad
C_\nu:=\overline{\operatorname{co}}^{\,g}(K_\nu),
\]
where \(\overline{\operatorname{co}}^{\,g}(K_\nu)\) denotes the closed geodesic
convex hull of \(K_\nu\).

\paragraph{Entropic barycentric transport map.}
Since \((\mathcal M,d)\) is a global NPC space, every probability measure in
\(\mathcal P_2(\mathcal M)\) admits a unique barycenter. For \(\varepsilon>0\),
disintegrate the entropic optimal plan as
\[
\pi_\varepsilon^\star(dx,dy)=\mu(dx)\,\pi_{\varepsilon,x}^\star(dy).
\]

\begin{proposition}[Entropic barycentric transport map]
\label{prop:entropic-bary-map}
For every \(\varepsilon>0\), the map
\[
T_\varepsilon(x):=\operatorname{bar}(\pi_{\varepsilon,x}^\star),
\qquad x\in K_\mu,
\]
is well defined for \(\mu\)-a.e.\ \(x\), Borel measurable, and takes values in
\(C_\nu\).
\end{proposition}

The proof is deferred to Appendix~\ref{app:proof-entropic-bary-map}.

\paragraph{Neural barycentric map.}
Let \(\mathcal G_m\subset C(K_\nu)\) be a neural hypothesis class and, for
\(\varepsilon>0\), let \(g_{m,\varepsilon}\in \mathcal G_m\). Define
\[
f_{m,\varepsilon}:=\mathcal T_\nu^\varepsilon g_{m,\varepsilon},
\]
and the induced Gibbs plan
\begin{equation}
\label{eq:neural-gibbs-plan-meps}
d\widehat\pi_{m,\varepsilon}(x,y)
:=
\exp\!\left(
\frac{f_{m,\varepsilon}(x)+g_{m,\varepsilon}(y)-c(x,y)}{\varepsilon}
\right)\,d\mu(x)d\nu(y).
\end{equation}
By construction, \(\widehat\pi_{m,\varepsilon}\) is a probability measure with
first marginal \(\mu\). Disintegrating with respect to \(\mu\),
\[
\widehat\pi_{m,\varepsilon}(dx,dy)
=
\mu(dx)\,\widehat\pi_{m,\varepsilon,x}(dy),
\]
we define the associated neural barycentric map
\[
\widehat T_{m,\varepsilon}(x)
:=
\operatorname{bar}(\widehat\pi_{m,\varepsilon,x}),
\qquad \mu\text{-a.e. }x.
\]

For convenience, define the semidual suboptimality gap
\begin{equation}
\label{eq:def-gap-meps}
\Delta_{m,\varepsilon}
:=
\mathcal J_\varepsilon(g_\varepsilon^\star)-\mathcal J_\varepsilon(g_{m,\varepsilon})
=
\mathrm{OT}_\varepsilon-\mathcal J_\varepsilon(g_{m,\varepsilon}).
\end{equation}

The next result shows that semidual near-optimality implies convergence of the
associated barycentric maps.

\begin{theorem}[Neural recovery of the entropic barycentric map]
\label{thm:neural-recovery-entropic-map}
Fix \(\varepsilon>0\), and let \((g_{m,\varepsilon})_{m\in\mathbb N}\) be a sequence
with \(g_{m,\varepsilon}\in\mathcal G_m\) such that
\[
\Delta_{m,\varepsilon}\xrightarrow[m\to\infty]{}0.
\]
Then
\[
\widehat\pi_{m,\varepsilon}\to \pi_\varepsilon^\star
\quad\text{in total variation},
\]
and
\[
\widehat T_{m,\varepsilon}\to T_\varepsilon
\quad\text{in }L^1(\mu)\text{ and }L^2(\mu).
\]
More precisely,
\begin{equation}
\label{eq:main-L1-map-bound-gap}
\int_{K_\mu}
d\bigl(\widehat T_{m,\varepsilon}(x),T_\varepsilon(x)\bigr)\,\mu(dx)
\le
D_\nu\sqrt{\frac{\Delta_{m,\varepsilon}}{2\varepsilon}},
\end{equation}
and
\begin{equation}
\label{eq:main-L2-map-bound-gap}
\int_{K_\mu}
d\bigl(\widehat T_{m,\varepsilon}(x),T_\varepsilon(x)\bigr)^2\,\mu(dx)
\le
2D_\nu^2\sqrt{\frac{\Delta_{m,\varepsilon}}{2\varepsilon}}.
\end{equation}
\end{theorem}

The proof is deferred to Appendix~\ref{app:proof-neural-recovery-entropic-map}.

\paragraph{Zero-temperature limit.}
We now relate the entropic barycentric maps \(T_\varepsilon\) to the
unregularized quadratic optimal transport map.

\begin{assumption}[Uniqueness and continuity of the Monge map]
\label{ass:continuous-monge}
The unregularized quadratic optimal transport problem between \(\mu\) and \(\nu\)
admits a unique optimal plan \(\pi^\star\), and this plan is induced by a Borel map
\(T:K_\mu\to K_\nu\):
\[
\pi^\star=(\mathrm{id},T)_\#\mu.
\]
Moreover, \(T\) admits a continuous version on \(K_\mu\), still denoted by \(T\).
\end{assumption}

\begin{remark}
A sufficient condition for the existence and \(\mu\)-a.e.\ uniqueness of the Monge
map is that \(\mu\) be absolutely continuous with respect to the Riemannian volume
measure. The additional continuity assumption is used only in the proof of
Theorem~\ref{thm:zero-temp-map}; it can be weakened by a Lusin-type approximation
argument, at the price of a longer proof.
\end{remark}

\begin{theorem}[Zero-temperature convergence of entropic barycentric maps]
\label{thm:zero-temp-map}
Assume Assumption~\ref{ass:continuous-monge}. Then
\[
T_\varepsilon\to T
\quad\text{in }L^2(\mu)
\qquad\text{as }\varepsilon\downarrow0.
\]
In particular,
\[
T_\varepsilon\to T
\quad\text{in }L^1(\mu).
\]
\end{theorem}

The proof is deferred to Appendix~\ref{app:proof-zero-temp-map}.

Finally, we combine the fixed-\(\varepsilon\) neural approximation with the
vanishing-regularization limit.

\begin{theorem}[Diagonal recovery of the unregularized optimal transport map]
\label{thm:diagonal-map}
Assume Assumption~\ref{ass:continuous-monge}. Let
\((\varepsilon_k)_{k\in\mathbb N}\) be any sequence such that
\(\varepsilon_k\downarrow0\). For each \(k\in\mathbb N\), let
\(g_{m_k,\varepsilon_k}\in\mathcal G_{m_k}\), and define
\[
\widehat T_{m_k,\varepsilon_k}(x)
:=
\operatorname{bar}(\widehat\pi_{m_k,\varepsilon_k,x}).
\]
If
\begin{equation}
\label{eq:diagonal-gap-condition}
\frac{\Delta_{m_k,\varepsilon_k}}{\varepsilon_k}\xrightarrow[k\to\infty]{}0,
\end{equation}
then
\[
\widehat T_{m_k,\varepsilon_k}\to T
\quad\text{in }L^1(\mu)\text{ and }L^2(\mu).
\]
\end{theorem}

The proof is deferred to Appendix~\ref{app:proof-diagonal-map}.

\begin{remark}[How to choose the diagonal sequence]
\label{rem:choose-diagonal}
Suppose that for every fixed \(\varepsilon>0\), the classes \(\mathcal G_m\) are
universal on \(K_\nu\) and training returns approximate semidual maximizers, so that
\[
\inf_{m\ge 1}\Delta_{m,\varepsilon}=0.
\]
Then for any prescribed sequence \(\varepsilon_k\downarrow0\), one may choose
\(m_k\) such that
\[
\Delta_{m_k,\varepsilon_k}\le \frac{\varepsilon_k}{k^2}.
\]
In that case \eqref{eq:diagonal-gap-condition} holds automatically, and
Theorem~\ref{thm:diagonal-map} applies.
\end{remark}


\paragraph{Recovering the OT Map on Compact Manifolds.}


\begin{theorem}[Diagonal recovery of the unregularized optimal transport map]
\label{thm:diagonal-map}
Assume Assumption~\ref{ass:continuous-monge}. Let $\varepsilon_k\downarrow0$ be any
sequence. For each $k$, choose $m_k\in\mathbb N$ and a neural potential
$g_{m_k,\varepsilon_k}\in \mathcal G_{m_k}$, and let
$\widehat T_{m_k,\varepsilon_k}$ be the associated neural barycentric map.

If
\begin{equation}
\label{eq:diagonal-gap-condition}
\frac{\Delta_{m_k,\varepsilon_k}}{\varepsilon_k}\longrightarrow 0,
\end{equation}
then
\[
\widehat T_{m_k,\varepsilon_k}\to T
\quad\text{in }L^1(\mu)\text{ and }L^2(\mu).
\]
In particular, the stronger condition
\[
\Delta_{m_k,\varepsilon_k}=o(\varepsilon_k)
\]
is sufficient.
\end{theorem}







\clearpage
\newpage

\paragraph{Implementing and Training ERNOT.}

Given a neural parameterization $g_\theta:K_\nu\to \mathbb R$, the natural optimization problem is
\begin{equation}
\label{eq:training-objective}
\mathcal L_\varepsilon(\theta)
:=
-\mathcal J_\varepsilon(g_\theta)
=
-\int_{K_\nu} g_\theta\,d\nu
-\int_{K_\mu}\mathcal T_\nu^\varepsilon g_\theta\,d\mu.
\end{equation}
Minimizing $\mathcal L_\varepsilon$ is equivalent to maximizing the entropic semidual over the neural hypothesis class.

\clearpage
\newpage




\subsection{Cartan--Hadamard barycentric projection and recovery of transport maps}
\label{sec:ch-barycentric-projection}

In this subsection we specialize to the case where $(\mathcal M,g)$ is a
Cartan--Hadamard manifold, i.e.\ a complete, simply connected Riemannian manifold
with nonpositive sectional curvature. We retain the notation of
Section~\ref{sec:eot-compact-supports}: the measures $\mu,\nu\in\mathcal P(\mathcal M)$
have compact supports
\[
K_\mu:=\operatorname{spt}(\mu),
\qquad
K_\nu:=\operatorname{spt}(\nu),
\]
the cost is
\[
c(x,y):=\frac12 d(x,y)^2,
\]
and, for each $\varepsilon>0$, the entropic optimal plan is denoted by
$\pi_\varepsilon^\star$ with Schr\"odinger potentials
$(f_\varepsilon^\star,g_\varepsilon^\star)$.

We further write
\[
D_\nu:=\operatorname{diam}(K_\nu)<\infty.
\]

\paragraph{Barycenters on Cartan--Hadamard manifolds.}
Since $(\mathcal M,d)$ is a global NPC space, every probability measure
$q\in \mathcal P_2(\mathcal M)$ admits a unique barycenter
\[
\operatorname{bar}(q)
:=
\arg\min_{z\in \mathcal M}\int_{\mathcal M} d(z,y)^2\,q(dy),
\]
and the barycenter map is $1$-Lipschitz from
$\bigl(\mathcal P_1(\mathcal M),W_1\bigr)$ to $(\mathcal M,d)$:
\[
d\bigl(\operatorname{bar}(p),\operatorname{bar}(q)\bigr)
\le
W_1(p,q),
\qquad
p,q\in \mathcal P_1(\mathcal M).
\]
Moreover, the barycenter satisfies the variance inequality
\begin{equation}
\label{eq:variance-ineq-bary}
\int_{\mathcal M} d(z,y)^2\,q(dy)
\ge
d\bigl(z,\operatorname{bar}(q)\bigr)^2
+
\int_{\mathcal M} d\bigl(\operatorname{bar}(q),y\bigr)^2\,q(dy),
\qquad z\in \mathcal M.
\end{equation}

\begin{proposition}[Entropic barycentric transport map]
\label{prop:entropic-bary-map}
For every $\varepsilon>0$, disintegrate the optimal entropic plan as
\[
\pi_\varepsilon^\star(dx,dy)=\mu(dx)\,\pi_{\varepsilon,x}^\star(dy).
\]
Then the map
\[
T_\varepsilon(x):=\operatorname{bar}(\pi_{\varepsilon,x}^\star),
\qquad x\in K_\mu,
\]
is well defined for $\mu$-a.e.\ $x$, Borel measurable, and takes values in the closed
geodesic convex hull of $K_\nu$.
\end{proposition}

\begin{proof}
Since $\pi_\varepsilon^\star$ is supported on $K_\mu\times K_\nu$, its conditional laws
$\pi_{\varepsilon,x}^\star$ are supported on $K_\nu$ for $\mu$-a.e.\ $x$. In particular
$\pi_{\varepsilon,x}^\star\in \mathcal P_2(\mathcal M)$, so the barycenter
$\operatorname{bar}(\pi_{\varepsilon,x}^\star)$ is well defined and unique.

The kernel $x\mapsto \pi_{\varepsilon,x}^\star$ is Borel measurable as a map from
$K_\mu$ into $\mathcal P(K_\nu)$ equipped with the weak topology. Since $K_\nu$ is
compact, the weak topology on $\mathcal P(K_\nu)$ coincides with the $W_1$-topology.
Because the barycenter map is $1$-Lipschitz for $W_1$, it is continuous; hence
$x\mapsto T_\varepsilon(x)$ is Borel measurable.

Finally, in a Cartan--Hadamard manifold the squared-distance barycenter belongs to
the closed geodesic convex hull of the support of the measure. Since
$\operatorname{spt}(\pi_{\varepsilon,x}^\star)\subset K_\nu$, the claim follows.
\end{proof}

\paragraph{Neural barycentric map.}
Let $\mathcal G_m\subset C(K_\nu)$ be a neural hypothesis class and, for
$\varepsilon>0$, let $g_{m,\varepsilon}\in \mathcal G_m$. Define
\[
f_{m,\varepsilon}:=\mathcal T_\nu^\varepsilon g_{m,\varepsilon},
\]
and the induced Gibbs measure
\begin{equation}
\label{eq:neural-gibbs-plan-meps}
d\widehat\pi_{m,\varepsilon}(x,y)
:=
\exp\!\left(
\frac{f_{m,\varepsilon}(x)+g_{m,\varepsilon}(y)-c(x,y)}{\varepsilon}
\right)\,d\mu(x)d\nu(y).
\end{equation}
By construction, $\widehat\pi_{m,\varepsilon}$ is a probability measure with first
marginal $\mu$. Disintegrating with respect to $\mu$,
\[
\widehat\pi_{m,\varepsilon}(dx,dy)
=
\mu(dx)\,\widehat\pi_{m,\varepsilon,x}(dy),
\]
we define the associated neural barycentric map
\[
\widehat T_{m,\varepsilon}(x)
:=
\operatorname{bar}(\widehat\pi_{m,\varepsilon,x}),
\qquad \mu\text{-a.e. }x.
\]

For convenience, define the semidual suboptimality gap
\begin{equation}
\label{eq:def-gap-meps}
\Delta_{m,\varepsilon}
:=
\mathcal J_\varepsilon(g_\varepsilon^\star)-\mathcal J_\varepsilon(g_{m,\varepsilon})
=
\mathrm{OT}_\varepsilon-\mathcal J_\varepsilon(g_{m,\varepsilon}).
\end{equation}

\begin{lemma}[Fiberwise total variation identity]
\label{lem:fiber-tv-identity}
Let $\pi,\widetilde\pi\in \mathcal P(K_\mu\times K_\nu)$ have first marginal $\mu$, and
write
\[
\pi(dx,dy)=\mu(dx)\,\pi_x(dy),
\qquad
\widetilde\pi(dx,dy)=\mu(dx)\,\widetilde\pi_x(dy).
\]
If total variation is defined by
\[
\|\rho-\widetilde\rho\|_{\mathrm{TV}}
:=
\frac12\int \bigl|d\rho-d\widetilde\rho\bigr|,
\]
then
\[
\|\pi-\widetilde\pi\|_{\mathrm{TV}}
=
\int_{K_\mu}\|\pi_x-\widetilde\pi_x\|_{\mathrm{TV}}\,\mu(dx).
\]
\end{lemma}

\begin{proof}
Let
\[
\lambda(dx,dy)
:=
\mu(dx)\bigl(\pi_x+\widetilde\pi_x\bigr)(dy).
\]
Then $\pi,\widetilde\pi\ll \lambda$, and
\[
\frac{d\pi}{d\lambda}(x,y)-\frac{d\widetilde\pi}{d\lambda}(x,y)
=
\frac{d\pi_x}{d(\pi_x+\widetilde\pi_x)}(y)
-
\frac{d\widetilde\pi_x}{d(\pi_x+\widetilde\pi_x)}(y)
\]
for $\mu$-a.e.\ $x$. Therefore
\begin{align*}
2\|\pi-\widetilde\pi\|_{\mathrm{TV}}
&=
\int_{K_\mu\times K_\nu}
\left|
\frac{d\pi}{d\lambda}-\frac{d\widetilde\pi}{d\lambda}
\right|\,d\lambda \\
&=
\int_{K_\mu}
\left(
\int_{K_\nu}
\left|
\frac{d\pi_x}{d(\pi_x+\widetilde\pi_x)}
-
\frac{d\widetilde\pi_x}{d(\pi_x+\widetilde\pi_x)}
\right|
\,d(\pi_x+\widetilde\pi_x)
\right)\mu(dx) \\
&=
2\int_{K_\mu}\|\pi_x-\widetilde\pi_x\|_{\mathrm{TV}}\,\mu(dx).
\end{align*}
\end{proof}

\begin{proposition}[From plan convergence to barycentric map convergence]
\label{prop:plan-to-map}
For every $m\in\mathbb N$ and $\varepsilon>0$,
\begin{equation}
\label{eq:L1-map-bound}
\int_{K_\mu}
d\bigl(\widehat T_{m,\varepsilon}(x),T_\varepsilon(x)\bigr)\,\mu(dx)
\le
D_\nu\,\|\widehat\pi_{m,\varepsilon}-\pi_\varepsilon^\star\|_{\mathrm{TV}}.
\end{equation}
Consequently,
\begin{equation}
\label{eq:L1-map-bound-gap}
\int_{K_\mu}
d\bigl(\widehat T_{m,\varepsilon}(x),T_\varepsilon(x)\bigr)\,\mu(dx)
\le
D_\nu
\sqrt{\frac{\Delta_{m,\varepsilon}}{2\varepsilon}}.
\end{equation}
Moreover,
\begin{equation}
\label{eq:L2-map-bound-gap}
\int_{K_\mu}
d\bigl(\widehat T_{m,\varepsilon}(x),T_\varepsilon(x)\bigr)^2\,\mu(dx)
\le
D_\nu^2
\sqrt{\frac{\Delta_{m,\varepsilon}}{2\varepsilon}}.
\end{equation}
\end{proposition}

\begin{proof}
By the $W_1$-contraction of the barycenter map,
\[
d\bigl(\widehat T_{m,\varepsilon}(x),T_\varepsilon(x)\bigr)
\le
W_1\!\bigl(\widehat\pi_{m,\varepsilon,x},\pi_{\varepsilon,x}^\star\bigr)
\qquad \mu\text{-a.e. }x.
\]
Since both measures are supported on $K_\nu$,
\[
W_1\!\bigl(\widehat\pi_{m,\varepsilon,x},\pi_{\varepsilon,x}^\star\bigr)
\le
D_\nu\,
\|\widehat\pi_{m,\varepsilon,x}-\pi_{\varepsilon,x}^\star\|_{\mathrm{TV}}.
\]
Integrating and using Lemma~\ref{lem:fiber-tv-identity} yields
\[
\int_{K_\mu}
d\bigl(\widehat T_{m,\varepsilon}(x),T_\varepsilon(x)\bigr)\,\mu(dx)
\le
D_\nu
\int_{K_\mu}
\|\widehat\pi_{m,\varepsilon,x}-\pi_{\varepsilon,x}^\star\|_{\mathrm{TV}}
\,\mu(dx)
=
D_\nu\,\|\widehat\pi_{m,\varepsilon}-\pi_\varepsilon^\star\|_{\mathrm{TV}}.
\]
This proves \eqref{eq:L1-map-bound}.

Next, Proposition~\ref{prop:dual-gap-kl} gives
\[
\varepsilon\,\mathrm{KL}\!\left(\pi_\varepsilon^\star\mid \widehat\pi_{m,\varepsilon}\right)
=
\Delta_{m,\varepsilon},
\]
and Pinsker's inequality yields
\[
\|\widehat\pi_{m,\varepsilon}-\pi_\varepsilon^\star\|_{\mathrm{TV}}
\le
\sqrt{\frac{\Delta_{m,\varepsilon}}{2\varepsilon}}.
\]
Combining with \eqref{eq:L1-map-bound} proves \eqref{eq:L1-map-bound-gap}.

Finally, since both barycentric maps take values in the closed convex hull of $K_\nu$,
their pointwise distance is bounded by $D_\nu$. Hence
\[
d\bigl(\widehat T_{m,\varepsilon}(x),T_\varepsilon(x)\bigr)^2
\le
D_\nu\,
d\bigl(\widehat T_{m,\varepsilon}(x),T_\varepsilon(x)\bigr),
\]
and integrating \eqref{eq:L1-map-bound-gap} gives \eqref{eq:L2-map-bound-gap}.
\end{proof}

\begin{theorem}[Neural recovery of the entropic barycentric map]
\label{thm:neural-recovery-entropic-map}
Assume the hypotheses of Theorem~\ref{thm:plan-convergence}. Then, for each fixed
$\varepsilon>0$,
\[
\widehat\pi_{m,\varepsilon}\to \pi_\varepsilon^\star
\quad\text{in total variation},
\]
and
\[
\widehat T_{m,\varepsilon}\to T_\varepsilon
\quad\text{in }L^1(\mu)\text{ and }L^2(\mu).
\]
More precisely,
\[
\int d\bigl(\widehat T_{m,\varepsilon},T_\varepsilon\bigr)\,d\mu
\le
D_\nu\sqrt{\frac{\Delta_{m,\varepsilon}}{2\varepsilon}},
\qquad
\int d\bigl(\widehat T_{m,\varepsilon},T_\varepsilon\bigr)^2\,d\mu
\le
D_\nu^2\sqrt{\frac{\Delta_{m,\varepsilon}}{2\varepsilon}}.
\]
\end{theorem}

\begin{proof}
The total variation convergence follows from
Theorem~\ref{thm:plan-convergence}. The stated $L^1$ and $L^2$ convergence bounds then
follow directly from Proposition~\ref{prop:plan-to-map}.
\end{proof}

\paragraph{Zero-temperature limit.}
We now relate the entropic barycentric maps $T_\varepsilon$ to the
unregularized quadratic optimal transport map.

\begin{assumption}[Uniqueness and continuity of the Monge map]
\label{ass:continuous-monge}
The unregularized quadratic OT problem between $\mu$ and $\nu$ admits a unique optimal
plan $\pi^\star$, and this plan is induced by a Borel map
$T:K_\mu\to K_\nu$:
\[
\pi^\star=(\mathrm{id},T)_\#\mu.
\]
Moreover, $T$ admits a continuous version on $K_\mu$, still denoted by $T$.
\end{assumption}

\begin{remark}
A sufficient condition for the existence and $\mu$-a.e.\ uniqueness of the Monge map is
that $\mu$ be absolutely continuous with respect to the Riemannian volume measure. The
additional continuity assumption is used only in the proof of
Theorem~\ref{thm:zero-temp-map}; it can be weakened by a Lusin-type approximation
argument, at the price of a longer proof.
\end{remark}

\begin{theorem}[Zero-temperature convergence of barycentric entropic maps]
\label{thm:zero-temp-map}
Assume Assumption~\ref{ass:continuous-monge}. Then
\[
T_\varepsilon\to T
\quad\text{in }L^2(\mu)
\qquad\text{as }\varepsilon\downarrow0.
\]
In particular, $T_\varepsilon\to T$ in $L^1(\mu)$.
\end{theorem}

\begin{proof}
By Theorem~5.10(c) of the entropic OT lecture notes, the entropic optimizers converge
weakly:
\[
\pi_\varepsilon^\star \Rightarrow \pi^\star=(\mathrm{id},T)_\#\mu
\qquad (\varepsilon\downarrow0).
\]
Since $T$ is continuous on the compact set $K_\mu$ and $K_\nu$ is compact, the function
\[
\Phi(x,y):=d\bigl(y,T(x)\bigr)^2
\]
is bounded and continuous on $K_\mu\times K_\nu$. Therefore weak convergence yields
\[
\iint_{K_\mu\times K_\nu}
d\bigl(y,T(x)\bigr)^2\,\pi_\varepsilon^\star(dx,dy)
\longrightarrow
\iint_{K_\mu\times K_\nu}
d\bigl(y,T(x)\bigr)^2\,\pi^\star(dx,dy)
=
0.
\]
Now fix $\varepsilon>0$ and disintegrate
\[
\pi_\varepsilon^\star(dx,dy)=\mu(dx)\,\pi_{\varepsilon,x}^\star(dy).
\]
Applying the barycenter variance inequality \eqref{eq:variance-ineq-bary} to the measure
$\pi_{\varepsilon,x}^\star$ with $z=T(x)$ gives, for $\mu$-a.e.\ $x$,
\[
d\bigl(T_\varepsilon(x),T(x)\bigr)^2
\le
\int_{K_\nu} d\bigl(y,T(x)\bigr)^2\,\pi_{\varepsilon,x}^\star(dy).
\]
Integrating in $x$ and using Fubini,
\[
\int_{K_\mu} d\bigl(T_\varepsilon(x),T(x)\bigr)^2\,\mu(dx)
\le
\iint_{K_\mu\times K_\nu}
d\bigl(y,T(x)\bigr)^2\,\pi_\varepsilon^\star(dx,dy)
\longrightarrow 0.
\]
This proves the $L^2(\mu)$ convergence.
\end{proof}



\begin{proof}
By Theorem~\ref{thm:neural-recovery-entropic-map},
\[
\int d\bigl(\widehat T_{m_k,\varepsilon_k},T_{\varepsilon_k}\bigr)\,d\mu
\le
D_\nu
\sqrt{\frac{\Delta_{m_k,\varepsilon_k}}{2\varepsilon_k}}
\longrightarrow 0.
\]
By Theorem~\ref{thm:zero-temp-map},
\[
\int d\bigl(T_{\varepsilon_k},T\bigr)^2\,d\mu\to0,
\]
hence also
\[
\int d\bigl(T_{\varepsilon_k},T\bigr)\,d\mu\to0.
\]
Therefore
\[
\int d\bigl(\widehat T_{m_k,\varepsilon_k},T\bigr)\,d\mu
\le
\int d\bigl(\widehat T_{m_k,\varepsilon_k},T_{\varepsilon_k}\bigr)\,d\mu
+
\int d\bigl(T_{\varepsilon_k},T\bigr)\,d\mu
\to0.
\]
This proves the $L^1(\mu)$ convergence.

Since all maps take values in the compact set $\overline{\mathrm{co}}^{\,g}(K_\nu)$,
their pointwise distance is bounded by $D_\nu$, so
\[
d\bigl(\widehat T_{m_k,\varepsilon_k}(x),T(x)\bigr)^2
\le
D_\nu\, d\bigl(\widehat T_{m_k,\varepsilon_k}(x),T(x)\bigr).
\]
Integrating and using the $L^1(\mu)$ convergence yields the $L^2(\mu)$ convergence.
\end{proof}

\begin{remark}[How to choose the diagonal sequence]
\label{rem:choose-diagonal}
Suppose that for every fixed $\varepsilon>0$, the classes $\mathcal G_m$ are universal on
$K_\nu$ and training returns approximate semidual maximizers, so that
\[
\inf_{m\ge 1}\Delta_{m,\varepsilon}=0.
\]
Then for any prescribed sequence $\varepsilon_k\downarrow0$ one may choose $m_k$ such that
\[
\Delta_{m_k,\varepsilon_k}\le \frac{\varepsilon_k}{k^2}.
\]
In that case \eqref{eq:diagonal-gap-condition} holds automatically, and
Theorem~\ref{thm:diagonal-map} applies.
\end{remark}

==> sections/related_work.tex <==
\paragraph{Optimal transport and entropic regularization.}
Optimal transport provides a geometric framework for comparing probability
measures and constructing couplings and maps between them
\citep{Villani2003,Villani2009,Santambrogio2015,PeyreCuturi2019}.
Entropic regularization turns discrete OT into a smooth problem that can be
solved efficiently by Sinkhorn scaling \citep{Cuturi2013}, and is closely
connected to the Schr\"odinger problem \citep{Leonard2014}. Sinkhorn and
semidual formulations are now widely used in machine learning, including
stochastic OT optimization \citep{GenevayCuturiPeyreBach2016},
differentiable Sinkhorn losses \citep{GenevayPeyreCuturi2018}, and debiased
Sinkhorn divergences \citep{FeydySejourneVialardAmariTrouvePeyre2019}. Our
work builds on this entropic OT perspective, but replaces the Euclidean
quadratic cost by the intrinsic quadratic geodesic cost on a Riemannian
manifold.

\paragraph{Optimal transport on Riemannian manifolds.}
Monge--Kantorovich transport extends naturally to curved spaces when the cost
is defined through the geodesic distance. For
\(c(x,y)=\frac12 d(x,y)^2\), the Riemannian analogue of Brenier's theorem
represents optimal maps using exponential maps of Kantorovich potentials
\citep{McCann2001}. Riemannian OT has also played an important role in
geometric inequalities and curvature-dimension theory
\citep{CorderoErausquinMcCannSchmuckenschlaeger2001,LottVillani2009,Sturm2006}.
The regularity of optimal maps is subtle because of curvature and cut-locus
effects \citep{Loeper2009,FigalliRiffordVillani2010}. Since our setting
includes non-compact manifolds, it is also related to work on Monge solutions
on complete non-compact manifolds \citep{FathiFigalli2007}. In contrast with
these mostly analytic works, our goal is computational: to learn entropic
transport plans and summaries from samples while respecting the intrinsic
geometry.


\paragraph{Neural optimal transport.}
Neural OT methods amortize the computation of maps or potentials using neural
networks. Early approaches learned a regularized OT plan and fitted a neural
map to its barycentric projection
\citep{SeguyDamodaranFlamaryCourtyRoletBlondel2018}. Other methods exploit
Euclidean Brenier structure by parameterizing convex potentials with
input-convex neural networks \citep{MakkuvaTaghvaeiOhLee2020}, or learn maps
and plans for more general costs and weak transport formulations
\citep{KorotinSelikhanovychBurnaev2023}. Entropic neural OT has also been
studied through dynamic Schr\"odinger bridge formulations
\citep{GushchinKolesovBurnaev2023}. Our work is closest to neural
potential-based OT, but defines the cost, soft \(c\)-transform, and transport
summaries intrinsically on a Riemannian manifold rather than in an ambient
Euclidean space.

\paragraph{Riemannian neural OT and manifold generative models.}
Recent generative models also operate directly on manifolds. Riemannian
score-based and diffusion models extend Euclidean diffusion models using
Brownian motion, Riemannian scores, or manifold SDEs
\citep{DeBortoliMathieuHutchinsonThorntonTehDoucet2022,
HuangAghajohariBosePanangadenCourville2022}, while Riemannian flow matching
learns geometry-aware continuous normalizing flows
\citep{ChenLipmanBenHamu2024}. These are generative modelling frameworks
rather than entropic OT semidual solvers, but they are related through their
use of intrinsic probability dynamics. Closest to our setting is recent work
on Riemannian Neural Optimal Transport, which studies continuous neural
parameterizations of manifold OT maps
\citep{MicheliCaoMonodBhatt2026}. Our work is complementary: we focus on the
entropic semidual formulation, heat-smoothed transport extraction, and
non-compact Riemannian manifolds such as Euclidean products, Lie groups, and
the SPD cone.
